Stellar Evolution in the Disks of Active Galactic Nuclei Produces Rapidly Rotating Massive Stars

Stars can either be formed in or captured by the accretion disks in Active Galactic Nuclei (AGN). These AGN stars are irradiated and subject to extreme levels of accretion, which can turn even low-mass stars into very massive ones ($M > 100 {\rm M}_\odot$) whose evolution may result in the formation of massive compact objects ($M > 10 {\rm M}_\odot$). Here we explore the spins of these AGN stars and the remnants they leave behind. We find that AGN stars rapidly spin up via accretion, eventually reaching near-critical rotation rates. They further maintain near-critical rotation even as they shed their envelopes, become compact, and undergo late stages of burning. This makes them good candidates to produce high-spin massive black holes, such as the ones seen by LIGO-Virgo in GW190521g, as well as long Gamma Ray Bursts (GRBs) and the associated chemical pollution of the AGN disk.

==> Snippets/constants.tex <==
%constants
\newcommand{\kB}{\ensuremath{k_\mathrm{B}}} %Boltzmann's constant
\newcommand{\NA}{\ensuremath{N_\mathrm{\!A}}} %Avogadro number
\newcommand{\mb}{\ensuremath{m_\mathrm{u}}} %mean nucleon mas
\newcommand{\me}{\ensuremath{m_\mathrm{e}}} %electron mass
\newcommand{\mpr}{\ensuremath{m_\mathrm{p}}} %proton mass
\newcommand{\mn}{\ensuremath{m_\mathrm{n}}} %neutron mass
\newcommand{\alphaF}{\ensuremath{\alpha_\mathrm{F}}} %Fine structure


==> Snippets/derivatives.tex <==
% $Id: derivatives.tex 385 2008-07-13 20:07:02Z efb $

%differential operators, roman typeface
\newcommand{\dif}{\ensuremath{\mathrm{d}}}
\newcommand{\Dif}{\ensuremath{\mathrm{D}}}

%derivatives
\newcommand{\D}{{\mathrm d}}
\newcommand{\DD}{{\,\D\!\!\;}}
\newcommand{\dd}[2]{\frac{\partial #1}{\partial #1}} %partialderivative 
\newcommand{\ddt}[1]{\frac{\partial #1}{\partial t}} %partial time derivative 
%\newcommand{\DDt}[1]{\frac{\dif #1}{\dif t}} %total time derivative
\newcommand{\DDt}[1]{\frac{\Dif #1}{\Dif t}} % Lagrangian time derivative
\newcommand{\ddm}[1]{\frac{\partial #1}{\partial m}} %partial derivative wrt m 
\newcommand{\ddr}[1]{\frac{\partial #1}{\partial r}} %partial derivative wrt r
\newcommand{\ddx}[1]{\frac{\partial #1}{\partial x}} %partial derivative wrt x 
\newcommand{\ddy}[1]{\frac{\partial #1}{\partial y}} %partial derivative wrt y 
\newcommand{\DDy}[1]{\frac{\dif #1}{\dif y}} %total derivative wrt y
\newcommand{\ddz}[1]{\frac{\partial #1}{\partial z}} %partial derivative wrt z 
\newcommand{\ppl}[2]{\left(\frac{\partial\ln #1}{\partial\ln
      #2}\right)_{\rho,T}}
\newcommand{\ppll}[2]{\left(\frac{\partial\ln #1}{\partial\ln
      #2}\right)_{\rho,T,\{X_{j\neq i}\}}}
\newcommand{\ddl}[2]{\frac{{\rm d}\ln #1}{{\rm d}\ln #2}}
\newcommand{\DxDy}[2]{{\frac{\D{#1}}{\D{#2}}}}
\newcommand{\dxdy}[2]{{\frac{\partial{#1}}{\partial{#2}}}}
\newcommand{\dxdyind}[3]{{\Brak{\frac{\D{#1}}{\D{#2}}}_{{#3}}}}
\newcommand{\dxdycz}[3]{{\Brak{\frac{\partial{#1}}{\partial{#2}}}_{{#3}}}}
%Misc
\newcommand{\Av}[1]{{\left\langle{#1}\right\rangle}}
\newcommand{\av}[1]{{\langle{#1}\rangle}}
\newcommand{\Frac}[2]{{\Brak{#1}/\Brak{#2}}}
\newcommand{\abs}[1]{{\left|{#1}\right|}}


==> Snippets/formatting.tex <==
%=======================================================================
%
% formatting.tex --- Formatting Macros
%
%=======================================================================

%References

\newcommand{\lSect}[1]{{\label{sec:#1}}}
\newcommand{\lFig}[1]{{\label{fig:#1}}}
\newcommand{\lEq}[1]{{\label{eq:#1}}}
\newcommand{\lTab}[1]{{\label{tab:#1}}}
\newcommand{\pFig}[1]{{\placefigure{fig:#1}}}
\newcommand{\pTab}[1]{{\placetable{tab:#1}}}
\newcommand{\Tabff}[1]{{\ref{tab:#1}}}
\newcommand{\Tab}[1]{{Table~\Tabff{#1}}}
\newcommand{\Tabs}[1]{{Tables~\Tabff{#1}}}
\newcommand{\TabRange}[2]{{Tables~\Tabff{#1} - \Tabff{#2}}}
\newcommand{\TabTwo}[2]{{Tables~\Tabff{#1} and \Tabff{#2}}}
\newcommand{\pan}[1]{{\textit{#1}}}
\newcommand{\Pan}[1]{{Panel~\pan{#1}}}
\newcommand{\Pans}[1]{{Panels~\pan{#1}}}
\newcommand{\FIGFF}[2]{{\ref{fig:#2}\pan{#1}}}
\newcommand{\Figff}[1]{{\FIGFF{}{#1}}}
\newcommand{\FIG}[2]{{Fig.~\FIGFF{#1}{#2}}}
\newcommand{\Fig}[1]{{\FIG{}{#1}}}
\newcommand{\FigTwo}[2]{{\FIGS{}{#1} and \FIGFF{}{#2}}}
\newcommand{\FIGS}[2]{{Figs.~\FIGFF{#1}{#2}}}
\newcommand{\Figs}[1]{{\FIGS{}{#1}}}
\newcommand{\Figure}[1]{{Figure~\FIGFF{}{#1}}}
\newcommand{\Figures}[1]{{Figures~\FIGFF{}{#1}}}
\newcommand{\Sectff}[1]{{\ref{sec:#1}}}
\newcommand{\Sect}[1]{{\S\Sectff{#1}}}
\newcommand{\Appendix}[1]{{Appendix~\Sectff{#1}}}
\newcommand{\Appendices}[1]{{Appendices~\Sectff{#1}}}
\newcommand{\Sects}[1]{{\S\S\Sectff{#1}}}
\newcommand{\Eqref}[1]{{\ref{eq:#1}}}
\newcommand{\Eqff}[1]{{(\Eqref{#1})}}
\newcommand{\EQ}[1]{{Equation~\Eqff{#1}}}
\newcommand{\Equation}[1]{{Equation~\Eqff{#1}}}
\newcommand{\Eq}[1]{{Eq.~\Eqff{#1}}}
\newcommand{\Eqs}[1]{{Eqs.~\Eqff{#1}}}
\newcommand{\Leg}[1]{{\textit{#1}}}

% formatting macros

\newcommand{\isofont}[1]{{\mathrm{#1}}}
\newcommand{\isomass}[1]{{\ensuremath{\isofont{^{#1}}}}}
\newcommand{\isocharge}[1]{{\ensuremath{\isofont{_{#1}}}}}
\newcommand{\isotope}[3]{{\ensuremath{\isocharge{#1}\isomass{#2}\isofont{#3}}}}
\newcommand{\Solar}[1]{{\ensuremath{\left[\right.}#1\ensuremath{\right.\left]}}}
\newcommand{\I}[2]{{\isotope{}{#1}{#2}}}
\newcommand{\El}[1]{{\I{}{#1}}}
\newcommand{\Rat}[4]{{\I{#1}{#2}/\I{#3}{#4}}}
\newcommand{\SolRatI}[4]{{\Solar{\Rat{#1}{#2}{#3}{#4}}}}
\newcommand{\SolI}[2]{{\Solar{\I{#1}{#2}}}} \newcommand{\SolEl}[1]{{\Solar{\El{#1}}}} 
\newcommand{\Ep}[1]{{\ensuremath{10^{#1}}}}
\newcommand{\E}[1]{{\ensuremath{\powersep\Ep{#1}}}}
\newcommand{\EE}[2]{{\ensuremath{\powersep\Ep{#1#2}}}}
\newcommand{\powersep}{\times}
\newcommand{\Brak}[1]{{\left({#1}\right)}}
\newcommand{\SBrak}[1]{{\left[{#1}\right]}}


==> Snippets/nuclides.tex <==
% $Id: nuclides.tex 385 2008-07-13 20:07:02Z efb $
% nuclides.tex
% input file with macros for nuclides

% base command
\newcommand{\nuclei}[2]{\ensuremath{\mathrm{^{#1}#2}}}

% nuclides, with most highest abundance or longest half-life as default
% for example, \carbon produces ^{12}C, \carbon[13] produces ^{13}C
%
\newcommand{\neutron}{\ensuremath{n}}
\newcommand{\nt}{\neutron}
\newcommand{\proton}{\ensuremath{p}}
\newcommand{\pt}{\proton}
\newcommand{\photon}{\ensuremath{\gamma}}
\newcommand{\hydrogen}[1][1]{\nuclei{#1}{H}}
\newcommand{\helium}[1][4]{\nuclei{#1}{He}}
\newcommand{\lithium}[1][7]{\nuclei{#1}{Li}}
\newcommand{\beryllium}[1][9]{\nuclei{#1}{Be}}
\newcommand{\boron}[1][11]{\nuclei{#1}{B}}
\newcommand{\carbon}[1][12]{\nuclei{#1}{C}}
\newcommand{\nitrogen}[1][14]{\nuclei{#1}{N}}
\newcommand{\oxygen}[1][16]{\nuclei{#1}{O}}
\newcommand{\fluorine}[1][19]{\nuclei{#1}{F}}
\newcommand{\neon}[1][20]{\nuclei{#1}{Ne}}
\newcommand{\sodium}[1][23]{\nuclei{#1}{Na}}
\newcommand{\magnesium}[1][24]{\nuclei{#1}{Mg}}
\newcommand{\aluminum}[1][27]{\nuclei{#1}{Al}}
\newcommand{\silicon}[1][28]{\nuclei{#1}{Si}}
\newcommand{\phosphorus}[1][31]{\nuclei{#1}{P}}
\newcommand{\sulfur}[1][32]{\nuclei{#1}{S}}
\newcommand{\chlorine}[1][35]{\nuclei{#1}{Cl}}
\newcommand{\argon}[1][36]{\nuclei{#1}{Ar}}
\newcommand{\potassium}[1][39]{\nuclei{#1}{K}}
\newcommand{\calcium}[1][40]{\nuclei{#1}{Ca}}
\newcommand{\scandium}[1][45]{\nuclei{#1}{Sc}}
\newcommand{\titanium}[1][48]{\nuclei{#1}{Ti}}
\newcommand{\vanadium}[1][51]{\nuclei{#1}{V}}
\newcommand{\chromium}[1][52]{\nuclei{#1}{Cr}}
\newcommand{\manganese}[1][55]{\nuclei{#1}{Mn}}
\newcommand{\iron}[1][56]{\nuclei{#1}{Fe}}
\newcommand{\cobalt}[1][59]{\nuclei{#1}{Co}}
\newcommand{\nickel}[1][58]{\nuclei{#1}{Ni}}
\newcommand{\copper}[1][63]{\nuclei{#1}{Cu}}
\newcommand{\zinc}[1][64]{\nuclei{#1}{Zn}}
\newcommand{\gallium}[1][69]{\nuclei{#1}{Ga}}
\newcommand{\germanium}[1][74]{\nuclei{#1}{Ge}}
\newcommand{\arsenic}[1][75]{\nuclei{#1}{As}}
\newcommand{\selenium}[1][80]{\nuclei{#1}{Se}}
\newcommand{\bromine}[1][79]{\nuclei{#1}{Br}}
\newcommand{\krypton}[1][84]{\nuclei{#1}{Kr}}
\newcommand{\rubidium}[1][85]{\nuclei{#1}{Rb}}
\newcommand{\strontium}[1][88]{\nuclei{#1}{Sr}}
\newcommand{\yttrium}[1][89]{\nuclei{#1}{Y}}
\newcommand{\zirconium}[1][94]{\nuclei{#1}{Zr}}
\newcommand{\niobium}[1][93]{\nuclei{#1}{Nb}}
\newcommand{\molybdenum}[1][98]{\nuclei{#1}{Mo}}
\newcommand{\technetium}[1][97]{\nuclei{#1}{Tc}}
\newcommand{\ruthenium}[1][102]{\nuclei{#1}{Ru}}
\newcommand{\rhodium}[1][103]{\nuclei{#1}{Rh }}
\newcommand{\palladium}[1][106]{\nuclei{#1}{Pd}}
\newcommand{\silver}[1][107]{\nuclei{#1}{Ag}}
\newcommand{\cadmium}[1][114]{\nuclei{#1}{Cd}}
\newcommand{\indium}[1][115]{\nuclei{#1}{In}}
\newcommand{\tin}[1][120]{\nuclei{#1}{Sn}}
\newcommand{\antimony}[1][121]{\nuclei{#1}{Sb}}
\newcommand{\tellurium}[1][130]{\nuclei{#1}{Te}}
\newcommand{\iodine}[1][127]{\nuclei{#1}{I}}
\newcommand{\xenon}[1][132]{\nuclei{#1}{Xe}}
\newcommand{\cesium}[1][133]{\nuclei{#1}{Cs}}
\newcommand{\barium}[1][138]{\nuclei{#1}{Ba}}
\newcommand{\lanthanum}[1][139]{\nuclei{#1}{La}}
\newcommand{\cerium}[1][140]{\nuclei{#1}{Ce}}
\newcommand{\praseodymium}[1][141]{\nuclei{#1}{Pr}}
\newcommand{\neodymium}[1][142]{\nuclei{#1}{Nd}}
\newcommand{\promethium}[1][147]{\nuclei{#1}{Pm}}
\newcommand{\samarium}[1][152]{\nuclei{#1}{Sm}}
\newcommand{\europium}[1][153]{\nuclei{#1}{Eu}}
\newcommand{\gadolinium}[1][158]{\nuclei{#1}{Gd}}
\newcommand{\terbium}[1][159]{\nuclei{#1}{Tb}}
\newcommand{\dysprosium}[1][164]{\nuclei{#1}{Dy}}
\newcommand{\holmium}[1][165]{\nuclei{#1}{Ho}}
\newcommand{\erbium}[1][168]{\nuclei{#1}{Er}}
\newcommand{\thulium}[1][169]{\nuclei{#1}{Tm}}
\newcommand{\ytterbium}[1][174]{\nuclei{#1}{Yb}}
\newcommand{\lutetium}[1][175]{\nuclei{#1}{Lu}}
\newcommand{\hafnium}[1][180]{\nuclei{#1}{Hf}}
\newcommand{\tantalum}[1][180]{\nuclei{#1}{Ta}}
\newcommand{\tungsten}[1][184]{\nuclei{#1}{W}}
\newcommand{\rhenium}[1][187]{\nuclei{#1}{Re}}
\newcommand{\osmium}[1][192]{\nuclei{#1}{Os}}
\newcommand{\iridium}[1][193]{\nuclei{#1}{Ir}}
\newcommand{\platnium}[1][195]{\nuclei{#1}{Pt}}
\newcommand{\gold}[1][197]{\nuclei{#1}{Au}}
\newcommand{\mercury}[1][202]{\nuclei{#1}{Hg}}
\newcommand{\thallium}[1][205]{\nuclei{#1}{Tl}}
\newcommand{\lead}[1][208]{\nuclei{#1}{Pb}}
\newcommand{\bisumth}[1][209]{\nuclei{#1}{Bi}}
\newcommand{\polonium}[1][210]{\nuclei{#1}{Po}}
\newcommand{\astatine}[1][210]{\nuclei{#1}{At}}
\newcommand{\radon}[1][222]{\nuclei{#1}{Rn}}
\newcommand{\francium}[1][223]{\nuclei{#1}{Fr}}
\newcommand{\radium}[1][226]{\nuclei{#1}{Ra}}
\newcommand{\actinium}[1][227]{\nuclei{#1}{Ac}}
\newcommand{\thorium}[1][232]{\nuclei{#1}{Th}}
\newcommand{\protactinium}[1][231]{\nuclei{#1}{Pa}}
\newcommand{\uranium}[1][238]{\nuclei{#1}{U}}
\newcommand{\neptunium}[1][237]{\nuclei{#1}{Np}}
\newcommand{\plutonium}[1][244]{\nuclei{#1}{Pu}}
\newcommand{\americium}[1][243]{\nuclei{#1}{Am}}
\newcommand{\curium}[1][247]{\nuclei{#1}{Cm}}
\newcommand{\berkelium}[1][247]{\nuclei{#1}{Bk}}
\newcommand{\californium}[1][251]{\nuclei{#1}{Cf}}
\newcommand{\einsteinium}[1][252]{\nuclei{#1}{Es}}
\newcommand{\fermium}[1][257]{\nuclei{#1}{Fm}}
\newcommand{\mendelevium}[1][258]{\nuclei{#1}{Md}}
\newcommand{\nobelium}[1][259]{\nuclei{#1}{No}}
\newcommand{\lawrencium}[1][262]{\nuclei{#1}{Lr}}
\newcommand{\rutherfordium}[1][261]{\nuclei{#1}{Rf}}
\newcommand{\dubnium}[1][268]{\nuclei{#1}{Db}}
\newcommand{\seaborgium}[1][271]{\nuclei{#1}{Sg}}
\newcommand{\bohrium}[1][274]{\nuclei{#1}{Bh}}
\newcommand{\hassium}[1][270]{\nuclei{#1}{Hs}}
\newcommand{\meitnerium}[1][278]{\nuclei{#1}{Mt}}
\newcommand{\darmstadtium}[1][281]{\nuclei{#1}{Ds}}
\newcommand{\roentgenium}[1][281]{\nuclei{#1}{Rg}}
\newcommand{\copernicum}[1][285]{\nuclei{#1}{Cn}}


==> Snippets/orcid.tex <==
0000-0001-5048-9973


==> Snippets/vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\bvec{\nabla} \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
% end vectors.tex

